A First Step Towards Detecting Values-violating Defects in Android APIs

Human values are an important aspect of life and should be supported in ubiquitous technologies such as mobile applications (apps). There has been a lot of focus on fixing certain kinds of violation of human values, especially privacy, accessibility, and security while other values such as pleasure, tradition, and humility have received little focus. In this paper, we investigate the relationship between human values and Android API services and developed algorithms to detect potential violation of these values. We evaluated our algorithms with a manually curated ground truthset resulting in a high performance, and applied the algorithms to 10,000 apps. Our results show a correlation between violation of values and the presence of viruses. Our results also show that apps with the lowest number of installations contain more violation of values and the frequency of the violation of values was highest in social apps.

==> pictures.tex <==


\section{Experimental result analysis}

\label{appendix:pictures}

this appendix contains all result analysis graphs with violation applications



\begin{figure}[t]
\label{fig:self direction and hedonism in android.media}
\includegraphics[width=0.5\textwidth]{media_sd.png}
\caption{Violations of self direction and hedonism in android.media by different category}
\centering
\end{figure}

\begin{figure}[H]
\label{fig:universalism in android.media}
\includegraphics[width=0.5\textwidth]{media_uni.png}
\caption{Violation of universalism in android.media by different category}
\centering
\end{figure}

\begin{figure}[H]
\label{fig:self direction in android.nfc}
\includegraphics[width=0.5\textwidth]{nfc_sd.png}
\caption{Violation of self direction in android.nfc by different category}
\centering
\end{figure}

\begin{figure}[H]
\label{fig:security in android.nfc}
\includegraphics[width=0.5\textwidth]{nfc_se.png}
\caption{Violation of security in android.nfc by different category}
\centering
\end{figure}

\begin{figure}[H]
\label{fig:ecurity and conformity in android.telephony}
\includegraphics[width=0.5\textwidth]{tele_se_confor.png}
\caption{Violation of security and conformity in android.telephony by different category}
\centering
\end{figure}

